Mapping Instructions and Visual Observations to Actions with Reinforcement Learning

We propose to directly map raw visual observations and text input to actions for instruction execution. While existing approaches assume access to structured environment representations or use a pipeline of separately trained models, we learn a single model to jointly reason about linguistic and visual input. We use reinforcement learning in a contextual bandit setting to train a neural network agent. To guide the agent's exploration, we use reward shaping with different forms of supervision. Our approach does not require intermediate representations, planning procedures, or training different models. We evaluate in a simulated environment, and show significant improvements over supervised learning and common reinforcement learning variants.

==> background.tex <==
\section{Background}
\label{sec:rl}

\paragraph{Reinforcement Learning} Reinforcement learning (RL) is a class of machine learning methods. In an RL setup, an agent learns to interact with a world to perform a specific task. For example, consider the <<EXAMPLE>>

The world is represented as a state s that describes the room, block location, and robot configuration. At each step, the robot performs an action a, for example pushing a block or moving.

The actions to be executed are selected according to a policy $\policy(\observ, \action)$. The execution of an action determines the next state of the world through a deterministic or probabilistic transition function. During learning, the agent receives a scalar reward after each action. The goal is to learn a policy that maximizes the expected total reward for all states, where the total reward is the sum of rewards received until the task completion. 

A key advantage of RL is its generalization potential. In contrast to supervised learning, where the learner is limited to the training data, the RL agent is not limited to observing a fixed subset of the state space. In addition, in RL, learning can rely on potentially weaker forms of supervision through the reward function, while supervised learning requires labeled data.

\paragraph{Deep Reinforcement Learning} In general, performance of RL methods is extremely sensitive to the state representation, which is often subject to various design assumptions and simplifications. In contrast, recent methods have suggested using deep neural networks to recover an expressive state representation [Mnih et al., 2013]. This approach is commonly referred to as deep RL, and has been shown to be effective for a broad set of tasks, including learning to play video games [Mnih et al., 2013], text-based games [Narasimhan et al., 2015], extracting information from the web [Narasimhan et al., 2016] and dialogue generation [Li et al., 2016].

\paragraph{Reinforcement Learning Challenges} RL methods present two common challenges. First, RL methods have been found to take a long time to learn a good policy. This is because RL methods, unlike supervised learning, do not rely on labeled training data and hence must explore the search space to learn a good policy. 

\paragraph{Reward Reshaping} Reward reshaping is a set of techniques for injecting prior knowledge into the reward function. Formally, reward reshaping converts a reward function $R$ into $R+F$ where $F:\statespace \times \actionspace \times \statespace \rightarrow \mathbb{R}$ is the reshaping term.

Adding an arbitrary reshaping term will change the problem and affect the total order of policies. It was shown by Ng et al. that if $F^a_{s,s'} = \gamma \phi(s') - \phi(s)$ for some potential function $\phi: \statespace \rightarrow \mathbb{R}$ then the total order of policies remains unchanged. This result was improved further by BLAH BLAH to show that using a potential function of the form $F^{a, a'}_{s, s'} = \gamma \phi(s', a') - \phi(s, a)$ keeps the total order of policy remains unchanged.
